Operational Resource Theory of Non-Markovianity

In order to analyze non-Markovianity of tripartite quantum states from a resource theoretical viewpoint, we introduce a class of quantum operations performed by three distant parties, and investigate an operational resource theory (ORT) induced it. A tripartite state is a free state if and only if it is a quantum Markov chain. We prove monotonicity of functions such as the conditional quantum mutual information, intrinsic information, squashed entanglement, a generalization of entanglement of purification, and the relative entropy of recovery. The ORT has five bound sets, each of which corresponds to one of the monotone functions. We introduce a task of "non-Markovianity dilution", and prove that the optimal rate for the task, namely the "non-Markovianity cost", is bounded from above by entanglement of purification in the case of pure states. We also propose a classical resource theory of non-Markovianity.

==> quantum resource theory/preferences.tex <==
%THEOREMS

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{thm}{ Theorem}
\newtheorem{dfn}[thm]{ Definition}
\newtheorem{lmm}[thm]{ Lemma}
\newtheorem{exa}[thm]{ Example}
\newtheorem{crl}[thm]{ Corollary}
\newtheorem{asm}[thm]{ Assumption}
\newtheorem{prp}[thm]{ Proposition}
\newtheorem{cjt}[thm]{ Conjecture}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{prf}{ Proof:}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{skprf}{ Sketch of the proof.}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{outprf}{ Outline of the proof.}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{prftyp}{ Proof of Theorem \ref{thm:typicalsubspace}.}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{prfconv}{ Proof of Theorem \ref{thm:misoptach}.}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{rmk}{ Remark.}}





%COMMANDS

\renewcommand{\theprf}{}
\renewcommand{\theprftyp}{}
\renewcommand{\theoutprf}{}
\renewcommand{\theprfconv}{}
\renewcommand{\thermk}{}
  

\newcommand{\bra}[1]{\mbox{$\langle#1|$}}
\newcommand{\Bra}[1]{\mbox{$\left\langle#1\right|$}}
\newcommand{\ket}[1]{\mbox{$|#1\rangle$}}
\newcommand{\Ket}[1]{\mbox{$\left|#1\right\rangle$}}
\newcommand{\inpro}[2]{\mbox{$\left\langle#1|#2\right\rangle$}}
\newcommand{\outpro}[2]{\mbox{$\ket{#1}\!\bra{#2}$}}
\newcommand{\Outpro}[2]{\mbox{$\Ket{#1}\!\Bra{#2}$}}
\newcommand{\proj}[1]{\mbox{$\ket{#1}\!\bra{#1}$}}
\newcommand{\Proj}[1]{\mbox{$\Ket{#1}\!\Bra{#1}$}}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\Norm}[1]{\left\|#1\right\|}
\newcommand{\kakko}[1]{\mbox{$\left(#1\right)$}}
\newcommand{\proof}{\noindent{\bf Proof.}  }
\newcommand{\ave}[1]{\mbox{$\left\langle#1\right\rangle$}}
\newcommand{\eq}[1]{Eq.(\ref{eq:#1})}
\newcommand{\sect}[1]{Sec.\,\ref{sec:#1}}
\newcommand{\ep}[1]{\noindent{\underline{\bf EP{#1}:}}}
\newcommand{\alg}[1]{\begin{align}#1\end{align}}
\newcommand{\rarrow}{\rightarrow}
\newcommand{\larrow}{\leftarrow}
\newcommand{\nn}{\nonumber}
\newcommand{\ca}[1]{{\mathcal #1}}
\newcommand{\Tr}[2]{{\rm Tr}_{#1}\left[#2\right]}
\newcommand{\bthm}[1]{\begin{thm}\label{thm:#1}}
\newcommand{\ethm}{\end{thm}}
\newcommand{\rthm}[1]{\ref{thm:#1}}
\newcommand{\rThm}[1]{Theorem \ref{thm:#1}}
\newcommand{\blmm}[1]{\begin{lmm}\label{lmm:#1}}
\newcommand{\elmm}{\end{lmm}}
\newcommand{\rLmm}[1]{Lemma \ref{lmm:#1}}
\newcommand{\rlmm}[1]{\ref{lmm:#1}}
\newcommand{\bdfn}[1]{\begin{dfn}\label{dfn:#1}}
\newcommand{\edfn}{\end{dfn}}
\newcommand{\rdfn}[1]{Definition \ref{dfn:#1}}
\newcommand{\bprp}[1]{\begin{prp}\label{prp:#1}}
\newcommand{\eprp}{\end{prp}}
\newcommand{\rprp}[1]{\ref{prp:#1}}
\newcommand{\rPrp}[1]{Proposition \ref{prp:#1}}
\newcommand{\bcrl}[1]{\begin{crl}\label{crl:#1}}
\newcommand{\ecrl}{\end{crl}}
\newcommand{\rcrl}[1]{Corollary \ref{crl:#1}}
\newcommand{\bprf}{\begin{prf}}
\newcommand{\eprf}{\end{prf}}
\newcommand{\brmk}{\begin{rmk}}
\newcommand{\ermk}{\end{rmk}}
\newcommand{\laeq}[1]{\label{eq:#1}}
\newcommand{\req}[1]{(\ref{eq:#1})}
\newcommand{\rineq}[1]{Inequality (\ref{eq:#1})}
\newcommand{\QED}{\hfill$\blacksquare$}
\newcommand{\lsec}[1]{\label{sec:#1}}
\newcommand{\rsec}[1]{\ref{sec:#1}}
\newcommand{\rSec}[1]{Section \ref{sec:#1}}
\newcommand{\lapp}[1]{\label{app:#1}}
\newcommand{\rapp}[1]{\ref{app:#1}}
\newcommand{\rApp}[1]{Appendix \ref{app:#1}}
\newcommand{\aR}{a_{\scalebox{0.45}{$R$}}}
\newcommand{\aL}{a_{\scalebox{0.45}{$L$}}}
\newcommand{\az}{a_{\scalebox{0.45}{$0$}}}
\newcommand{\bR}{b_{\scalebox{0.45}{$R$}}}
\newcommand{\bL}{b_{\scalebox{0.45}{$L$}}}
\newcommand{\bz}{b_{\scalebox{0.45}{$0$}}}
\newcommand{\baR}{{\bar a}_{\scalebox{0.45}{$R$}}}
\newcommand{\baL}{{\bar a}_{\scalebox{0.45}{$L$}}}
\newcommand{\baz}{{\bar a}_{\scalebox{0.45}{$0$}}}
\newcommand{\bbR}{{\bar b}_{\scalebox{0.45}{$R$}}}
\newcommand{\bbL}{{\bar b}_{\scalebox{0.45}{$L$}}}
\newcommand{\bbz}{{\bar b}_{\scalebox{0.45}{$0$}}}
\newcommand{\conv}{{\rm conv}}
\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}
\newcommand{\notations}{\noindent{\it Notations.} }
\newcommand{\bitem}{\begin{itemize}}
\newcommand{\entem}{\end{itemize}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\ennum}{\end{enumerate}}
\newcommand{\bb}{\mathbb}
\newcommand{\otm}{\otimes}
\newcommand{\opl}{\oplus}
\newcommand{\vro}{\varrho}
\newcommand{\rFig}[1]{Figure \ref{fig:#1}}
\newcommand{\rfig}[1]{\ref{fig:#1}}
\newcommand{\SH}{\noindent{\red [START HERE]} }


 
